B Physics at the Tevatron: Run II and Beyond

This report provides a comprehensive overview of the prospects for B physics at the Tevatron. The work was carried out during a series of workshops starting in September 1999. There were four working groups: 1) CP Violation, 2) Rare and Semileptonic Decays, 3) Mixing and Lifetimes, 4) Production, Fragmentation and Spectroscopy. The report also includes introductory chapters on theoretical and experimental tools emphasizing aspects of B physics specific to hadron colliders, as well as overviews of the CDF, D0, and BTeV detectors, and a Summary.

==> ch6/Bdk_D0.tex <==
\subsection{$B \ra D K$: D\O\ Report}

No report provided to date.



==> ch6/Bpsieta_D0.tex <==
\subsection{$B_s^0\ra J/\psi\eta^{(\prime)}$: D\O\ Report}

No report provided to date.



==> ch9/sec1/d0_style.tex <==
% D0 Style Definitions
% Definitions of commonly used symbols
%
% particles
\def\pbar{$\overline{p}$}               %pbar
  \def\tbar{$\overline{t}$}               %tbar
\def\bbar{$\overline{b}$}               %bbar
\def\pizero{$\pi^0$}                    %pizero
      \def\jpsi{$J/\psi$}                     %J/psi
\def\ppbar{$p\overline{p} $}            %ppbar
\def\pbarp{$\overline{p}p $}            %pbarp
\def\qqbar{$q\overline{q}$}             %qqbar
            \def\ttbar{$t\overline{t}$}             %ttbar
\def\bbbar{$b\overline{b}$}             %bbbar
\def\epm{$e^+e^-$}                      %e+e-
\def\wino{$\widetilde W$}               %Wino
\def\zino{$\widetilde Z$}               %Zino
\def\squark{$\widetilde q$}             %squark
\def\gluino{$\widetilde g$}             %gluino
%
% kinematics, physics quantities, etc.
\def\pt{$p_T$}                          %pT
\def\et{$E_T$}                          %ET
\def\ptrel{$P_T^{rel}$}			%PtRel
\def\met{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_T$}} %missing ET
\def\htran{$H_T$}                       %HT
\def\aplan{$\cal{A}$}                   %aplanarity
\def\iso{$\cal{I}$}                     %isolation variable
\def\remu{${\cal{R}}_{e\mu}$}           %distance between e and mu in eta-phi
\def\rmu{$\Delta\cal{R}_{\mu}$}         %distance between mu and jet cone axis
\def\sigtot{$\sigma_{\rm tot}$}         %sigma total
\def\sigtop{$\sigma_{t \overline{t}}$}  %sigma_ttbar
\def\njet{$N_{\rm jet}$}                %N_jet
\def\sinthw{sin$^2 \theta_W$}           %sin^2 th_W
\def\alphas{$\alpha_{\scriptscriptstyle S}$}                %alpha_s
\def\alphaem{$\alpha_{\scriptscriptstyle{\rm EM}}$}         %alpha_EM
%
% units
\def\ipb{pb$^{-1}$}                     %inverse picobarns
\def\gevcc{$GeV/c^2$}                   %GeV/c^2
\def\gevc{$GeV/c$}                        %GeV/c
\def\gev{$GeV$}                           %GeV
\def\deg{$^\circ$}                      %degree sign
%
% luminosity stuff
\def\lum{$\cal{L}$}                     %luminosity
\def\lumint{$\int\! {\cal{L}} dt$}      %integrated luminosity
\def\lumunits{cm$^{-2}$s$^{-1}$}        %luminosity units
%
% masses
\def\mt{$m_t$}                          %m_top 
\def\mb{$m_b$}                          %m_bottom
\def\mw{$M_W$}                          %M_W
\def\mz{$M_Z$}                          %M_Z
%
% misc.
\def\D0{D\O}                            %D0
\def\etal{{\sl et al.}}                 %et al. - no preceeding comma
\def\vs{{\sl vs.}}                      %vs. 
\def\d0draft{\special{header=draft.ps}}
\def\into{\rightarrow}                
%
%%
%%  References help:  DO NOT USE THESE FOR PAPERS WHICH WILL BE SUBMITTED
%%                               TO PRL OR PRD!!!!!!!!!!
%%
\newcommand{\NC}{{\em Nuovo Cimento\/} }
\newcommand{\NIM}{{\em Nucl. Instr. Meth.} }
\newcommand{\NP}{{\em Nucl. Phys.} }
\newcommand{\PL}{{\em Phys. Lett.} }
\newcommand{\PR}{{\em Phys. Rev.} }
\renewcommand{\PRL}{{\em Phys. Rev. Lett.} }
\newcommand{\RMP}{{\em Rev. Mod. Phys.} }
\newcommand{\ZP}{{\em Zeit. Phys.} }
% Parameters for references:
% parameter 1 - volume, parameter 2 - page, parameter 3- last two digits of year
\def\err#1#2#3 {{\it Erratum} {\bf#1},{\ #2} (19#3)}
\def\ib#1#2#3 {{\it ibid.} {\bf#1},{\ #2} (19#3)}
\def\nc#1#2#3 {Nuovo Cim. {\bf#1} ,#2(19#3)}
\def\nim#1#2#3 {Nucl. Instr. Meth. {\bf#1},{\ #2} (19#3)}
\def\np#1#2#3 {Nucl. Phys. {\bf#1},{\ #2} (19#3)}
\def\pl#1#2#3 {Phys. Lett. {\bf#1},{\ #2} (19#3)}
\def\prev#1#2#3 {Phys. Rev. {\bf#1},{\ #2} (19#3)}
\def\prl#1#2#3 {Phys. Rev. Lett. {\bf#1},{\ #2} (19#3)}
\def\rmp#1#2#3 {Rev. Mod. Phys. {\bf#1},{\ #2} (19#3)}
\def\zp#1#2#3 {Zeit. Phys. {\bf#1},{\ #2} (19#3)}

